Problem Theory

The Turing machine, as it was presented by Turing himself, models the calculations done by a person. This means that we can compute whatever any Turing machine can compute, and therefore we are Turing complete. The question addressed here is why, Why are we Turing complete? Being Turing complete also means that somehow our brain implements the function that a universal Turing machine implements. The point is that evolution achieved Turing completeness, and then the explanation should be evolutionary, but our explanation is mathematical. The trick is to introduce a mathematical theory of problems, under the basic assumption that solving more problems provides more survival opportunities. So we build a problem theory by fusing set and computing theories. Then we construct a series of resolvers, where each resolver is defined by its computing capacity, that exhibits the following property: all problems solved by a resolver are also solved by the next resolver in the series if certain condition is satisfied. The last of the conditions is to be Turing complete. This series defines a resolvers hierarchy that could be seen as a framework for the evolution of cognition. Then the answer to our question would be: to solve most problems. By the way, the problem theory defines adaptation, perception, and learning, and it shows that there are just three ways to resolve any problem: routine, trial, and analogy. And, most importantly, this theory demonstrates how problems can be used to found mathematics and computing on biology.

==> fonts.tex <==
% FONTS.TEX (RMCG19940923)

\catcode`\@=11

% Adaptado de pdcfsel.tex (v 3.5, 1995/03/28) by P. Damian Cugley

\def\expcs#1#2{\expandafter#1\csname#2\endcsname}
\def\noexpcs{\expcs\noexpand}

\def\loadfont#1#2{\ifx#1\relax \FSELloadfont#1{#2}\else
 \ifx#1\UNDEFINED \FSELloadfont#1{#2}\fi\fi}

\def\FSELloadfont#1#2{\edef#1{\global\font\noexpand#1#2\relax\noexpand#1}}

\def\xfontset#1#2#3{
    \def\f##1##2{\expcs\loadfont{#1##1}{##2#3}}
    \let\m=\f \let\M=\f
    \def\@##1##2##3{\expcs\loadfont{#1##2}{##3 at #3pt }}
    #2 }

\def\fontset#1#2#3#4#5#6{\xfontset{#1}{#2}{#3}%
    \expcs\edef{#1fonts}{%
       \noexpcs{#1mathsfonts}%
       \noexpand\FSELnicknames{#1}{#5}{#6}\noexpand#2%
       \noexpand\setbaselineskip{#4}%
       \noexpand\rm }%
       \expcs\def{#1mathsfonts}{\FSELloadmaths{#1}{#5}{#6}#2}}

\def\FSELnicknames#1#2#3{\let\@\relax
    \def\f##1##2{\expcs\edef{##1}{\noexpcs{#1##1}}}%
    \def\m##1##2{%
       \expcs\textfont{##1fam}\csname#1##1\endcsname
       \expcs\scriptfont{##1fam}\csname#2##1\endcsname
       \expcs\edef{##1}{%
           \fam\expcs\noexpand{##1fam}%
           \expcs\noexpand{#1##1}}}%
    \def\M##1{\expcs\scriptscriptfont{##1fam}\csname#3##1\endcsname
       \m{##1}}}

\def\setbaselineskip#1{\ifdim #1=\baselineskip \else
    \baselineskip#1\relax \normalbaselineskip\baselineskip
    \jot0.25\baselineskip
    \smallskipamount 0.25\baselineskip plus 0.083\baselineskip
       minus 0.083\baselineskip
    \medskipamount 0.5\baselineskip plus 0.167\baselineskip
       minus 0.167\baselineskip
    \bigskipamount 1\baselineskip plus 0.333\baselineskip
       minus 0.333\baselineskip
    \setbox\strutbox=\hbox{\vrule height 0.708\baselineskip
       depth 0.292\baselineskip width\z@}%
    \def\big##1{{\hbox{$\left##1\vbox to0.708\baselineskip
       {}\right.\n@space$}}}%
    \def\Big##1{{\hbox{$\left##1\vbox to0.958\baselineskip
       {}\right.\n@space$}}}%
    \def\bigg##1{{\hbox{$\left##1\vbox to1.208\baselineskip
       {}\right.\n@space$}}}%
    \def\Bigg##1{{\hbox{$\left##1\vbox to1.458\baselineskip
       {}\right.\n@space$}}}%
    \topskip=0.833\baselineskip \splittopskip=\topskip
    \abovedisplayskip=1\baselineskip
       plus0.25\baselineskip minus0.75\baselineskip
    \abovedisplayshortskip=0pt plus0.25\baselineskip
    \belowdisplayskip=\abovedisplayskip
    \belowdisplayshortskip=0.583\baselineskip
       plus0.25\baselineskip minus0.333\baselineskip
 \fi}

\def\FSELloadmaths#1#2#3{%
    \let\@\relax \def\f##1##2{}%
    \def\m##1##2{\csname#1##1\endcsname \csname#2##1\endcsname}%
    \def\M##1{\csname#3##1\endcsname \m{##1}}%
    \global\expcs\let{#1mathsfonts}\relax}

\chardef\rmfam=0 \chardef\mifam=1 \chardef\syfam=2

% Databases

\def\cmtemplate{%
   \M{rm}{cmr}\m{it}{cmti}\M{bf}{cmbx}\f{sc}{cmcsc}%
   \f{sl}{cmsl}\f{tt}{cmtt}\M{mi}{cmmi}\M{sy}{cmsy}}
\xfontset{cmscriptscript}\cmtemplate{5}
\xfontset{cmscript}\cmtemplate{7}
\fontset{cm}\cmtemplate{10}{12pt}{cmscript}{cmscriptscript}

\def\viiitemplate{%
   \m{rm}{cmr}\f{it}{cmti}\m{bf}{cmbx}%
   \f{sl}{cmsl}\f{tt}{cmtt}\m{mi}{cmmi}\m{sy}{cmsy}}
\xfontset{viiiscript}\viiitemplate{6}
\fontset{viii}\viiitemplate{8}{10pt}{viiiscript}{viiiscript}

\def\xiitemplate{%
   \M{rm}{cmr}\m{it}{cmti}\M{bf}{cmbx}\f{sc}{cmcsc}%
   \f{sl}{cmsl}\f{tt}{cmtt}\M{mi}{cmmi}\M{sy}{cmsy}}
\loadfont\xiisc{cmcsc10 at 12pt }
\loadfont\xiisy{cmsy10 at 12pt }
\xfontset{xiiscriptscript}\xiitemplate{6}
\xfontset{xiiscript}\xiitemplate{9}
\fontset{xii}\xiitemplate{12}{14.4pt}{xiiscript}{xiiscriptscript}

\def\xiibtemplate{%
   \M{rm}{cmr}\@\m{it}{cmbxti10}\M{bf}{cmbx}\@\f{sc}{cmssbx12}%
   \@\f{sl}{cmbxsl10}\@\f{tt}{cmtt12}\@\m{mi}{cmmib10}\@\m{sy}{cmbsy10}}
\xfontset{xiibscriptscript}\xiibtemplate{6}
\xfontset{xiibscript}\xiibtemplate{9}
\fontset{xiib}\xiibtemplate{12}{14.4pt}{xiibscript}{xiibscript}

\def\xivtemplate{%
   \M{rm}{cmr}\m{it}{cmti}\M{bf}{cmbx}\f{sc}{cmcsc}%
   \m{sl}{cmsl}\m{tt}{cmtt}\M{mi}{cmmi}\M{sy}{cmsy}}
\loadfont\xivrm{cmr12 at 14.4pt }
\loadfont\xivit{cmti12 at 14.4pt }
\loadfont\xivbf{cmbx12 at 14.4pt }
\loadfont\xivsc{cmcsc10 at 14.4pt }
\loadfont\xivsl{cmsl12 at 14.4pt }
\loadfont\xivtt{cmtt12 at 14.4pt }
\loadfont\xivmi{cmmi12 at 14.4pt }
\loadfont\xivsy{cmsy10 at 14.4pt }
\xfontset{xivscript}\xivtemplate{10}
\xfontset{xivscriptscript}\xivtemplate{7}
\fontset{xiv}\xivtemplate{14.28}{17pt}{xivscript}{xivscriptscript}

\def\xivbtemplate{%
   \@\m{rm}{cmr12}\@\m{it}{cmbxti10}\@\m{bf}{cmbx12}\@\f{sc}{cmr12}%
   \@\m{sl}{cmbxsl10}\@\m{tt}{cmtt12}\@\m{mi}{cmmib10}\@\m{sy}{cmbsy10}}
\xfontset{xivbscript}\xivbtemplate{7}
\fontset{xivb}\xivbtemplate{14.28}{17pt}{xivbscript}{xivbscript}

\def\xviitemplate{%
   \@\m{rm}{cmr12}\@\m{it}{cmti12}\@\m{bf}{cmbx12}\@\f{sc}{cmcsc10}%
   \@\m{sl}{cmsl12}\@\m{tt}{cmtt12}\@\m{mi}{cmmi12}\@\m{sy}{cmsy10}}
\xfontset{xviiscript}\xviitemplate{12}
\fontset{xvii}\xviitemplate{17.28}{21pt}{xviiscript}{xviiscript}

\def\xviibtemplate{%
   \@\m{rm}{cmbx12}\@\m{it}{cmbxti10}\@\m{bf}{cmbx12}\@\f{sc}{cmr17}%
   \@\m{sl}{cmbxsl10}\@\m{tt}{cmtt12}\@\m{mi}{cmmib10}\@\m{sy}{cmbsy10}}
\xfontset{xviibscript}\xviibtemplate{12}
\fontset{xviib}\xviibtemplate{17.28}{21pt}{xviibscript}{xviibscript}

\def\xxitemplate{%
   \@\m{rm}{cmr12}\@\m{it}{cmti12}\@\m{bf}{cmbx12}\@\f{sc}{cmcsc10}%
   \@\m{sl}{cmsl12}\@\m{tt}{cmtt12}\@\m{mi}{cmmi12}\@\m{sy}{cmsy10}}
\xfontset{xxiscript}\xxitemplate{14.28}
\fontset{xxi}\xxitemplate{20.736}{25pt}{xxiscript}{xxiscript}

\def\lmtemplate{%
   \M{rm}{texnansi-lmr}\m{it}{texnansi-lmri}%
   \M{bf}{texnansi-lmbx}\@\f{sc}{texnansi-lmcsc10}%
   \f{sl}{texnansi-lmro}\f{tt}{texnansi-lmtt}%
   \f{sf}{texnansi-lmss}\M{mi}{cmmi}\M{sy}{cmsy}}
\fontset{lm}\lmtemplate{10}{12pt}{cmscript}{cmscriptscript}

\loadfont\lmxiisy{cmsy10 at 12pt }
\fontset{lmxii}\lmtemplate{12}{14.4pt}{xiiscript}{xiiscriptscript}
\fontset{lmix}\lmtemplate{9}{11pt}{cmscript}{cmscriptscript}

\def\lmviiitemplate{%
   \m{rm}{texnansi-lmr}\f{it}{texnansi-lmri}%
   \m{bf}{texnansi-lmbx}\@\f{sc}{texnansi-lmcsc10}%
   \f{sl}{texnansi-lmro}\f{tt}{texnansi-lmtt}%
   \f{sf}{texnansi-lmss}\m{mi}{cmmi}\m{sy}{cmsy}}
\fontset{lmviii}\lmviiitemplate{8}{10pt}{viiiscript}{viiiscript}

\loadfont\lmxiizero{texnansi-lmr17 at 21pt }
\loadfont\lmxiione{texnansi-lmbx12 at 17pt }
\loadfont\lmxiitwo{texnansi-lmbx12 at 14.4pt }
\loadfont\lmzero{texnansi-lmr17}
\loadfont\lmone{texnansi-lmbx12 at 14.4pt }
\loadfont\lmtwo{texnansi-lmbx12}
\def\lmtitles{\def\fontzero{\lmzero}%
 \def\fontone{\lmone}\def\fonttwo{\lmtwo}}
\def\lmxiititles{\def\fontzero{\lmxiizero}%
 \def\fontone{\lmxiione}\def\fonttwo{\lmxiitwo}}

\def\pstemplate{%
   \@\M{rm}{ptmr8r}\@\M{it}{ptmri8r}\@\M{bf}{ptmb8r}\@\f{sc}{ptmrc8t}%
   \@\M{mi}{ptmri8t}\@\M{tt}{pcrr8r}}
\xfontset{psxscriptscript}\pstemplate{5}
\xfontset{psxscript}\pstemplate{7}
\fontset{psx}\pstemplate{10}{12pt}{psxscript}{psxscriptscript}

\xfontset{psxiiscriptscript}\pstemplate{6}
\xfontset{psxiiscript}\pstemplate{9}
\fontset{psxii}\pstemplate{12}{14.4pt}{psxiiscript}{psxiiscriptscript}

\xfontset{psxivscriptscript}\pstemplate{7}
\xfontset{psxivscript}\pstemplate{11}
\fontset{psxiv}\pstemplate{14.4}{17.28pt}{psxivscript}{psxivscriptscript}

\xfontset{psxviiscriptscript}\pstemplate{9}
\xfontset{psxviiscript}\pstemplate{14}
\fontset{psxvii}\pstemplate{17}{21pt}{psxviiscript}{psxviiscriptscript}

\xfontset{psxxiscriptscript}\pstemplate{10}
\xfontset{psxxiscript}\pstemplate{14}
\fontset{psxxi}\pstemplate{21}{25pt}{psxxiscript}{psxxiscriptscript}

\def\zerotemplate{\M{rm}{cmr}\M{it}{cmti}\M{bf}{cmbx}\M{sl}{cmsl}%
   \M{tt}{cmtt}}
\loadfont\zerobf{cmbx12 at 17.28pt }
\loadfont\zeroit{cmti12 at 17.28pt }
\loadfont\zerosl{cmsl12 at 17.28pt }
\loadfont\zerott{cmtt12 at 17.28pt }
\xfontset{zeroscriptscript}\zerotemplate{9}
\xfontset{zeroscript}\zerotemplate{12}
\fontset{zero}\zerotemplate{17}{20.4pt}{zeroscript}{zeroscriptscript}

\def\onetemplate{\M{rm}{cmr}\M{it}{cmti}\M{bf}{cmbx}\m{sl}{cmsl}%
   \m{tt}{cmtt}}
\loadfont\onerm{cmr12 at 14.4pt }
\loadfont\onebf{cmbx12 at 14.4pt }
\loadfont\oneit{cmti12 at 14.4pt }
\loadfont\onesl{cmsl12 at 14.4pt }
\loadfont\onett{cmtt12 at 14.4pt }
\xfontset{onescriptscript}\onetemplate{7}
\xfontset{onescript}\onetemplate{10}
\fontset{one}\onetemplate{14.4}{17.28pt}{onescript}{onescriptscript}

% Fonts for titles

\def\cmtitles{%
 \def\fontzero{\xviifonts\rm}%
 \def\fontone{\xivfonts\bf}%
 \def\fonttwo{\xiifonts\bf}%
}
\def\viiititles{%
 \def\fontzero{\xivfonts\bf}%
 \def\fontone{\xiifonts\bf}%
 \def\fonttwo{\cmfonts\bf}%
}
\def\xiititles{%
 \def\fontzero{\xxifonts\rm}%
 \def\fontone{\xviibfonts\bf}%
 \def\fonttwo{\xivbfonts\bf}%
 \def\fontthree{\xiibfonts\bf}%
}
\def\psxtitles{%
 \def\fontzero{\psxviifonts\rm}%
 \def\fontone{\psxivfonts\bf}%
 \def\fonttwo{\psxiifonts\bf}%
}
\def\psxiititles{%
 \def\fontzero{\psxxifonts\rm}%
 \def\fontone{\psxviifonts\bf}%
 \def\fonttwo{\psxivfonts\bf}%
}
\cmtitles

\catcode`\@=12

\endinput


==> index.tex <==
% index.tex (RMCG19931103)

\catcode`\@=11

\catcode`\^^02=12 \catcode`\^^03=12 \catcode`\^^04=12 \catcode`\^^05=12

% Check files auxiliar.aux, auxiliar.ind

\newread\infile

\newif\ifauxf
\openin\infile=auxiliar.aux
\ifeof\infile \auxffalse \else \auxftrue \fi
\closein\infile

\newif\ifindf
\openin\infile=auxiliar.ind
\ifeof\infile \indffalse \else \indftrue \fi
\closein\infile

% pdftex

\ifx\pdfoutput\undefined \csname newcount\endcsname\pdfoutput \fi

% \color{Red} ... \endcolor

\def\cmykWhite{0 0 0 0} \def\cmykDarkWhite{0 0 0 .3}
\def\cmykGray{0 0 0 .5} \def\cmykDarkGray{0 0 0 .7}
\def\cmykBlack{0 0 0 1} \def\cmykDarkBlack{.4 .3 .3 1}
\def\cmykYellow{0 0 1 0} \def\cmykDarkYellow{0 0 1 .7}
\def\cmykMagenta{0 1 0 0} \def\cmykDarkMagenta{0 1 0 .7}
\def\cmykCyan{1 0 0 0} \def\cmykDarkCyan{1 0 0 .7}
\def\cmykRed{0 1 1 0} \def\cmykDarkRed{0 1 1 .7}
\def\cmykGreen{1 0 1 0} \def\cmykDarkGreen{1 0 1 .7}
\def\cmykBlue{1 1 0 0} \def\cmykDarkBlue{1 1 0 .7}

\newcount\col@rstack
\def\pdf@color#1{\pdfcolorstack\col@rstack push {\csname cmyk#1\endcsname k}}
 \def\pdf@darkcolor#1{\pdfcolorstack\col@rstack push {\csname cmykDark#1\endcsname k}}
 \def\pdf@endcolor{\pdfcolorstack\col@rstack pop}
 \def\pdf@black{\pdfcolorstack\col@rstack push {0 g}}
\def\dvips@color#1{\special{color push cmyk \csname cmyk#1\endcsname}}
 \def\dvips@darkcolor#1{\special{color push cmyk \csname cmykDark#1\endcsname}}
 \def\dvips@endcolor{\special{color pop}}
 \def\dvips@black{\special{color push gray 0}}
\def\dvipdf@color#1{\special{pdf: bc [\csname cmyk#1\endcsname]}}
 \def\dvipdf@darkcolor#1{\special{pdf: bc [\csname cmykDark#1\endcsname]}}
 \def\dvipdf@endcolor{\special{pdf: ec}}
 \def\dvipdf@black{\special{pdf: bc [0]}}

\ifcase\pdfoutput
 \ifx\dvips\undefined
  \special{pdf: sc [0]}\let\colorblack=\dvipdf@black
  \def\colors{\let\color=\dvipdf@color\let\truecolor=\dvipdf@color\let\endcolor=\dvipdf@endcolor}
  \def\darkcolors{\let\color=\dvipdf@darkcolor\let\truecolor=\dvipdf@color\let\endcolor=\dvipdf@endcolor}
 \else
  \special{color gray 0}\let\colorblack=\dvips@black
  \def\colors{\let\color=\dvips@color\let\truecolor=\dvips@color\let\endcolor=\dvips@endcolor}
  \def\darkcolors{\let\color=\dvips@darkcolor\let\truecolor=\dvips@color\let\endcolor=\dvips@endcolor}
 \fi
\else
 \col@rstack=\pdfcolorstackinit page {0 g}\let\colorblack=\pdf@black
 \def\colors{\let\color=\pdf@color\let\truecolor=\pdf@color\let\endcolor=\pdf@endcolor}
 \def\darkcolors{\let\color=\pdf@darkcolor\let\truecolor=\pdf@color\let\endcolor=\pdf@endcolor}
\fi

\def\nocolor{\def\color##1{\relax}\def\truecolor##1{\relax}\def\endcolor{\relax}}
\nocolor % default value, \darkcolors intermediate with \colors

% type of links

\def\numlink#1{num \number#1}
\def\namelink#1{name {(\number#1)}}
\ifx\xmpinclude\undefined \let\typelink=\numlink \else \let\typelink=\namelink \fi

% \goto{Text in red}{123}

{\catcode`\#=12 \xdef\hash{#}}

\def\pdf@goto#1#2{\leavevmode
 \pdfstartlink attr{/F 4 /Border [0 0 0]} goto \typelink{#2}%
 \color{Red}#1\endcolor\pdfendlink\relax}
\def\dvips@goto#1#2{\leavevmode
 \special{html:<a href=\string"\hash\typelink{#2}\string">}%
 \color{Red}#1\endcolor\special{html:</a>}\relax}
\def\dvipdf@goto#1#2{\leavevmode
 \special{pdf: bann << /Type /Annot /Subtype /Link /Border [0 0 0]
   /A << /S /GoTo /D (\typelink{#2}) >> >>}\color{Red}#1\endcolor
 \special{pdf: eann}\relax}
\def\nolinks@goto#1#2{\leavevmode
 \closeout-1\color{Red}#1\endcolor\closeout-1\relax}
%\closeout-1 is just a whatsit, i.e. an extension as pdf commands are

% \dest

\newcount\d@stno

\def\pdf@dest{\global\advance\d@stno1
 \ifvmode \pdfdest \typelink{\d@stno} fitbh\else
  \vbox to0pt{\vss\pdfdest \typelink{\d@stno} fitbh\kern1pc}\fi}
\def\dvips@dest{\global\advance\d@stno1
 \ifvmode \special{html:<a name=\string"\typelink{\d@stno}\string">}
          \special{html:</a>}\else
  \vbox to0pt{\vss\special{html:<a name=\string"\typelink{\d@stno}\string">}
                  \special{html:</a>}\kern1pc}\fi}
\def\dvipdf@dest{\global\advance\d@stno1
 \ifvmode
  \special{pdf: dest (\typelink{\d@stno}) [@thispage /FitBH @ypos]}\else
  \vbox to0pt{\vss
   \special{pdf: dest (\typelink{\d@stno}) [@thispage /FitBH @ypos]}\kern1pc}\fi}
\def\nolinks@dest{\global\advance\d@stno1
 \ifvmode \closeout-1\else \vbox to0pt{\vss\closeout-1\kern1pc}\fi}

\ifcase\pdfoutput
 %\def\pdfcode#1\pdfendcode{\relax\closeout-1\relax}
 \ifx\dvips\undefined
  \def\links{\let\goto=\dvipdf@goto\let\dest=\dvipdf@dest}
 \else
  \def\links{\let\goto=\dvips@goto\let\dest=\dvips@dest}
 \fi
\else
 %\let\pdfcode=\relax \let\pdfendcode=\relax
 \def\links{\let\goto=\pdf@goto\let\dest=\pdf@dest}
\fi

\def\nolinks{\let\goto=\nolinks@goto\let\dest=\noliks@dest}
\links % default value

% \footnote

\def\footnoteoptions{} % \eightpt, for example
% adapted from [363]; parameter #2 (the text) is read later
\def\footnote#1{\let\@sf\empty
  \ifhmode\edef\@sf{\spacefactor\the\spacefactor}\/\fi
  \global\advance\d@stno1 \goto{#1}{\number\d@stno}\global\advance\d@stno-1% RMCG
  \@sf\vfootnote{#1}}
\def\vfootnote#1{\insert\footins\bgroup
  \interlinepenalty\interfootnotelinepenalty
  \splittopskip\ht\strutbox % top baseline for broken footnotes
  \splitmaxdepth\dp\strutbox \floatingpenalty\@MM
  \leftskip\z@skip \rightskip\z@skip \spaceskip\z@skip \xspaceskip\z@skip
  \footnoteoptions \textindent{#1}\footstrut\dest\futurelet\next\fo@t} % RMCG

% \pdf@ut calculates the number of branches in \@utno

\newtoks\pdft@k \pdft@k{}
\def\pdft@toc#1{\global\pdft@k=\expandafter{\the\pdft@k#1}}
\newcount\@utno \newcount\@uts
\newcount\@utss \newcount\@utt
\def\c@rcdr#1#2,{\edef\car{#1}\edef\cdr{#2}\ifx\cdr\empty\edef\cdr{0}\fi}
\def\pdf@ut{\expandafter\c@rcdr\the\pdft@k,\@uts=\car
 \global\pdft@k=\expandafter{\cdr}\toks0=\expandafter{\cdr}%
 \@utno=0 \@utss=\car \advance\@utss1
 \loop \expandafter\c@rcdr\the\toks0,\@utt=\car\toks0=\expandafter{\cdr}%
  \ifnum\@uts<\@utt \ifnum\@utss=\@utt\advance\@utno1\fi \repeat}

% Indexing

\def\ref#1{??} \def\refsc#1{??} \def\refpg#1{??}
% \toc{level}{text} \pdftocline{text}{\d@stno}
\let\toc=\gobbletwo \let\pdftocline=\gobbletwo
% \lbl{mnemonic}{replacement} \ndx{text}{type}
\let\lbl=\gobbletwo \let\ndx=\gobbletwo

% \pdfout{level}{title}{secid}
\def\pdfout#1#2#3{\if*#3#2\else#3 #2\fi}
\def\pdfoutA#1#2#3{#3 #2}
\def\pdfoutB#1#2#3{#2}

\def\pdf@outline#1#2#3#4#5{\ifnum#1<9
 \def\4{#4}\ifx\4\empty \let\pdfout=\pdfoutB \else \let\pdfout=\pdfoutA \fi
  {\stringate\doaccents\dosymbols\def\S{^^a7}\stringaccents \pdf@ut
   \pdfoutline goto \typelink{#3} count \number\@utno
               {\pdfout{#1}{#2}{#4}}}\fi}
\def\dvips@outline#1#2#3#4#5{\ifnum#1<9
 \def\4{#4}\ifx\4\empty \let\pdfout=\pdfoutB \else \let\pdfout=\pdfoutA \fi
 {\stringate\doaccents\dosymbols\def\S{^^a7}\stringaccents \pdf@ut
  \special{ps: [ /Title (\pdfout{#1}{#2}{#4}) /Count \number\@utno
   /Page #5 /OUT pdfmark}}\fi}
\def\dvipdf@outline#1#2#3#4#5{\ifnum#1<9
 \def\4{#4}\ifx\4\empty \let\pdfout=\pdfoutB \else \let\pdfout=\pdfoutA \fi
 {\stringate\doaccents\dosymbols\def\S{^^a7}\stringaccents \pdf@ut
  \special{pdf: out #1 << /Title (\pdfout{#1}{#2}{#4})
   /Dest (\typelink{#3}) >>}}\fi}

\def\fourdigits#1{\ifnum#1<0 \errmessage{min is 0}\else
            \ifnum#1>9999 \errmessage{max is 9999}\else
 \ifnum#1<1000 0\fi \ifnum#1<100 0\fi \ifnum#1<10 0\fi\fi\fi \number#1}
\ifx\secid\undefined \let\secid\empty\fi

\def\save#1{{\def\\{\string\\}\def~{\string~}\def\S{\string\S}\stringaccents
  \stringate\dohigh \deactivate\dohigh \utf\utf@Ch \let^^c2\empty
  \edef\next{\write\auxf{#1\string{\fourdigits\d@stno\string}%
    \string{\secid\string}\string{\noexpand\folio\string}}}\next}}

\newwrite\auxf \newwrite\tocf \newwrite\ndxf

\def\files{\begingroup \stringate\dohigh\stringaccents \let^^c2\empty
 \def~{\string~}\def\\{\string\\}\def\S{\string\S}\def\&{\string\&}% \catcode`\@=11
 \def\ftoc##1##2##3##4##5{\ifnum##1<9\pdft@toc{##1}\fi
  \immediate\write\tocf{\string\tocline
   \string{##1\string}\string{##2\string}%
   \string{##3\string}\string{##4\string}\string{##5\string}}}
 \def\fndx##1##2##3##4##5{\immediate\write\ndxf{\string\ndxline
  \string{##1\string}\string{##2\string}%
  \string{##3\string}\string{##4\string}\string{##5\string}}}
 \def\flbl##1##2##3##4##5{\setbox0=\hbox{\csname ^^03##1\endcsname}%
  \ifdim\wd0=0pt
   \expandafter\gdef\csname ^^02##1\endcsname{##2}% replacement
   \expandafter\gdef\csname ^^03##1\endcsname{##3}% \d@stno
   \expandafter\gdef\csname ^^04##1\endcsname{##4}% \secid
   \expandafter\gdef\csname ^^05##1\endcsname{##5}% \folio
  \else\errmessage{label ##1 redefined}\fi}
 \ifauxf
  \immediate\openout\tocf=auxiliar.toc
  \immediate\openout\ndxf=auxiliar.ind
  \input auxiliar.aux
  \immediate\closeout\tocf \immediate\closeout\ndxf
  \pdft@toc0
  \ifcase\pdfoutput
   \ifx\dvips\undefined \let\tocline=\dvipdf@outline
   \else \let\tocline=\dvips@outline\fi
  \else \let\tocline=\pdf@outline \fi
  \input auxiliar.toc
 \fi
 \endgroup
 \openout\auxf=auxiliar.aux
 \def\ref{\r@f^^02}\def\refsc{\r@f^^04}\def\refpg{\r@f^^05}%
 \def\toc##1##2{\save{\string\ftoc\string{##1\string}\string{##2\string}}}%
 \def\lbl##1##2{\save{\string\flbl\string{##1\string}\string{##2\string}}}%
 \def\ndx##1##2{\save{\string\fndx\string{##1\string}\string{##2\string}}}%
}
% Note that \vbox{}someword or someword\vbox{} does not hyphenate someword.

\def\r@f#1#2{{\stringate\dohigh\stringaccents\def\&{\string\&}\utf\utf@Ch \let^^c2\empty
  \xdef\n@@{\string"#2\string" }\xdef\@@n{\csname ^^03#2\endcsname}%
  \expandafter\global\expandafter\let\expandafter\@n@\csname #1#2\endcsname}%
 \setbox0=\hbox{\@n@}\ifdim\wd0=0pt ?\ifauxf\errmessage{label \n@@ undefined}\fi
  \else\goto{\@n@}{\@@n}\fi}

\def\label#1#2{\dest\lbl{#1}{#2}}
\def\index#1#2{\dest\ndx{#1}{#2}}

\catcode`\@=12

